ADAPTive Input Training for Many-to-One Pre-Training on Time-Series Classification

Recent work on time-series models has leveraged self-supervised training to learn meaningful features and patterns in order to improve performance on downstream tasks and generalize to unseen modalities. While these pretraining methods have shown great promise in one-to-many scenarios, where a model is pre-trained on one dataset and fine-tuned on a downstream dataset, they have struggled to generalize to new datasets when more datasets are added during pre-training. This is a fundamental challenge in building foundation models for time-series data, as it limits the ability to develop models that can learn from a large variety of diverse datasets available. To address this challenge, we present a new pre-training paradigm for time-series data called ADAPT, which can efficiently align the physical properties of data in the time-series domain, enabling mixed-batch pre-training despite the extreme discrepancies in the input sizes and channel dimensions of pre-training data. We trained on 162 time-series classification datasets and set new state-of-the-art performance for classification benchmarks. We successfully train a model within the time-series domain on a wide range of datasets simultaneously, which is a major building block for building generalist foundation models in time-series domains.

==> Main_Results.tex <==
\begin{longtable}[t]{lllll}
\toprule
\multirow{2}{*}{Model Name} & \multicolumn{4}{c}{Performance Metrics [\%]} \\ \cmidrule(lr){2-5}
                            & Accuracy & Precision & Recall & F1 Score\\ 
\midrule
\multicolumn{5}{c}{\textbf{Dataset: FD-B}} \\
\midrule[0.1pt](lr)
     TS-SD &  55.66±2.10 &   57.1±5.35 &  60.54±2.72 &  57.03±3.28 \\
    TS2vec &  47.9±1.13 &  43.39±0.92 &  48.42±1.97 &  43.89±1.07 \\
     CLOCS &  49.27±3.10 &  48.24±3.16 &  58.73±3.87 &  47.46±4.85 \\
 Mixing-up & 67.89±2.46 &  71.46±3.43 &  76.13±1.98 &  72.73±2.28 \\
    TS-TCC &  54.99±2.20 &  52.79±2.93 &  63.96±1.78 &  54.18±3.38 \\
    SimCLR & 49.17±4.37 & 54.46±10.24 &   47.60±8.85 & 42.24±11.38 \\
      TF-C & 69.38±2.31 &  75.59±3.49 &  72.02±2.57 &  74.87±2.68 \\
ADAPT(EEG) & 97.31±2.76 &  98.18±1.81 &  98.03±2.02 &  98.02±2.03 \\
     ADAPT & 91.21±4.21 &  90.97±4.08 &  91.77±4.20 &  88.76±5.73  \\
\midrule
\multicolumn{5}{c}{\textbf{Dataset: Gesture}} \\
\midrule[0.1pt](lr)
     TS-SD & 69.22±4.44 &  66.98±4.72 &  68.67±4.88 &  66.56±4.43  \\
    TS2vec & 69.17±3.33 &  65.45±3.58 &  68.54±3.49 &   65.70±3.92 \\
     CLOCS & 44.33±5.18 &  42.37±7.94 &  44.33±5.18 &  40.14±6.02 \\
 Mixing-up & 69.33±2.31 &  67.19±2.32 &  69.33±2.31 &  64.97±3.06 \\
    TS-TCC & 71.88±3.49 &  71.35±3.52 &  71.67±3.73 &   69.84±3.60 \\
    SimCLR & 48.04±5.94 & 59.46±16.23 & 54.11±19.46 &  49.55±18.70 \\
      TF-C & 76.42±1.96 &  77.31±3.55 &  74.29±2.68 &  75.72±3.11 \\
ADAPT(EEG) &  72.5±1.18 &  70.79±0.78 &   72.5±1.18 &  70.70±0.71 \\
     ADAPT &  77.00±2.50 &  74.85±3.74 &  77.00±2.51 &  75.05±2.94 \\
\midrule
\multicolumn{5}{c}{\textbf{Dataset: EMG}} \\
\midrule[0.1pt](lr)
     TS-SD &    46.06±0.00 &     15.45±0.00 &     33.33±0.00 &     21.11±0.00 \\
    TS2vec & 78.54±3.18 &    80.4±7.50 &  67.85±3.96 &  67.66±5.01\\
     CLOCS & 69.85±3.23 &   53.06±7.50 &  53.54±2.91 &  51.39±4.09 \\
 Mixing-up & 30.24±5.34 &  10.99±1.26 &  25.83±4.56 &  15.41±2.04 \\
    TS-TCC & 78.89±1.92 &  58.51±9.74 &   63.10±9.91 &  59.04±9.52 \\
    SimCLR & 61.46±5.82 & 53.61±17.24 &  49.9±12.14 & 47.08±14.86 \\
      TF-C & 81.71±2.87 &  72.65±3.53 &  81.59±2.89 &  76.83±3.11 \\
ADAPT(EEG) & 96.58±4.52 &  94.44±6.08 &  97.25±3.63 &  95.01±6.20 \\
     ADAPT & 98.54±1.19 &  96.66±2.72 &  98.82±0.96 &  97.58±1.98 \\
\midrule
\caption{Overall classification accuracy of ADAPT compared to other state-of-the-art pre-trained models for time-series classification. Baseline implementations are from \cite{Zhang2022Self-SupervisedConsistency} and we follow their implementation. All of the other baselines are pretrained on the SleepEEG dataset as it was the largest and most complex of the pretraining datasets. ADAPT enables mixed batch pretraining over any dataset within the time-series domain and therefore we can train one model across all of the pre-training datasets. We pre-train two models, ADAPT(EEG) which is only pre-trained on the SleepEEG datasets, and ADAPT which is trained on all of the pretraining datasets in Section 5.2. Our results indicate that ADAPT shows strong improvements in most categories, particularly on the FD-B and EMG datasets.}
\label{table:ClassificationResults}
\end{longtable}



==> inDomain.tex <==
\begin{longtable}{lllll}
\toprule
\multirow{2}{*}{Model Name} & \multicolumn{4}{c}{Performance Metrics [\%]} \\ \cmidrule(lr){2-5}
                            & Accuracy & Precision & Recall & F1 Score\\ 
\midrule
\multicolumn{5}{c}{\textbf{Dataset: Epilepsy}} \\
\midrule[0.1pt](lr)
     TS-SD & 89.52±5.22 & 80.18±22.44 & 76.47±14.85 & 77.67±18.55 \\
    TS2vec & 93.95±0.44 &  90.59±1.16 &  90.39±1.18 &  90.45±0.67 \\
     CLOCS & 95.07±0.27 &  93.01±0.67 &  91.27±1.65 &  92.06±0.66\\
 Mixing-up &    80.21±0 &     40.11±0 &        50±0 &     44.51±0 \\
    TS-TCC & 92.53±0.98 &  94.51±0.49 &  81.81±2.57 &  86.33±2.15 \\
    SimCLR & 90.71±3.44 &  92.21±1.66 & 78.64±10.71 &  81.78±9.98 \\
      TF-C & 94.95±2.49 &  94.56±1.08 &  89.08±2.16 &  91.49±5.34 \\
ADAPT(EEG) & 88.64±3.48 &  82.15±4.19 &  91.05±1.60 &  84.83±3.93 \\
     ADAPT & 93.63±2.95 &  90.13±4.90 & 91.73±0.91 &  88.53±4.65 \\
\caption{Results on in-domain classification between our model and current state-of-the-art baselines. Each model except ADAPT was pre-trained on the SleepEEG\cite{Sleep-EDFV1.0.0} dataset. ADAPT shows comparable performance with state-of-the-art models on in-domain classification and the mixed-batch training actually improves ADAPT's performance compared to the ADAPT(EEG) which was trained only on the SleepEEG dataset.}
\label{table:InDomainResults}
\end{longtable}
